Do autoencoders need a bottleneck for anomaly detection?

A common belief in designing deep autoencoders (AEs), a type of unsupervised neural network, is that a bottleneck is required to prevent learning the identity function. Learning the identity function renders the AEs useless for anomaly detection. In this work, we challenge this limiting belief and investigate the value of non-bottlenecked AEs. The bottleneck can be removed in two ways: (1) overparameterising the latent layer, and (2) introducing skip connections. However, limited works have reported on the use of one of the ways. For the first time, we carry out extensive experiments covering various combinations of bottleneck removal schemes, types of AEs and datasets. In addition, we propose the infinitely-wide AEs as an extreme example of non-bottlenecked AEs. Their improvement over the baseline implies learning the identity function is not trivial as previously assumed. Moreover, we find that non-bottlenecked architectures (highest AUROC=0.857) can outperform their bottlenecked counterparts (highest AUROC=0.696) on the popular task of CIFAR (inliers) vs SVHN (anomalies), among other tasks, shedding light on the potential of developing non-bottlenecked AEs for improving anomaly detection.

==> depracated/body_20220119.tex <==
% TODO:
% Get base from the STRATH report
% All datasets: +ODDS datasets 
% results and discussion 
% related work
% experiment setup
% Connection to GP: Infinite BAE


% \section{Do AEs need a bottleneck?}

\section{Introduction}


Extant work claims that AEs will trivially learn the identity mapping ($f_{\theta}(\textbf{x}) = \textbf{x}$) when no constraints are placed on it \cite{ruff2018, ng2011sparse}. In such cases, AEs will perfectly reconstruct any inputs (regardless whether it is anomalous or not), and hence the negative log-likelihood (or reconstruction loss) will be low for all inputs and this leads to unreliable anomaly detection. To prevent this, it is common to impose a bottleneck in the architecture, resulting in an undercomplete architecture; the output of the encoder has much lower dimensions than the input (i.e. $\text{dim}(f_\text{encoder}(\textbf{x}))<\text{dim}(\textbf{x})$). Nonetheless, most works analogically describe the need for a bottleneck and report the empirical performance of AEs with a bottleneck did not compare against AEs without bottleneck \cite{chen2018autoencoder, chow2020, kim2020, mujeeb2019, ruff2018}. 

\textbf{How do we eliminate the bottleneck?} There are two ways to eliminate the bottleneck: (1) simply expand the size of the latent dimensions to be equal to or greater than the flattened input dimensions, also known as an overcomplete architecture, and (2) introduce long-range skip connections from the encoder to the decoder akin to a U-Net architecture \cite{unet2015}, thereby allowing each layer's data flow to bypass the bottleneck. Implementing either or both of these design choices removes the bottleneck from the architecture; for clarity, we tabulate architectures which are and are not bottlenecked in Table XX. 

% make a figure

\begin{table}[hbtp]
\centering
    \begin{tabular}{ccc}
    \hline
    Architecture type & Latent dimensions & Skip connections \\ \hline
    \textbf{With bottleneck} &  &  \\
    A & Undercomplete & \xmark \\ \hline
    \textbf{Without bottleneck} &  &  \\
    B & Undercomplete & \cmark \\
    C & Overcomplete & \xmark \\
    D & Overcomplete & \cmark \\ \hline
    \end{tabular}
\end{table}
% why skip connections?
\textbf{Why skip connections?} Skip connections allow better flow of information in NNs with many layers leading to a smoother loss landscape \cite{li2017visualizing} and easier optimisation without additional computational complexity \cite{he2016deep}. Recently, \cite{collin2021, kim2021} reported that AEs with skip connections outperform those without on image anomaly detection. To prevent learning the identity mapping, \cite{collin2021} trained the AEs to output clean images out of noisy images (also known as denoising AEs). One challenge of modelling such denoising AEs for anomaly detection is the choice of synthetic corruption method, also known as data augmentation, which largely depends on the type of data (e.g. image, tabular, time-series, etc.) and type of expected anomalies (e.g. stained images) making it not easily generalisable to other data types.  
% Nonetheless, the use of skip connections in AE is not common for anomaly detection as it is assumed to promote learning the identity mapping.

% [put a picture here]
% Our work differs by finding that even without the denoising scheme, AEs with skip connections are unable to learn the identity function and may still perform well for anomaly detection. Moreover, our work attempts to shed light on a broader issue of whether AEs need bottlenecks at all.

Surprisingly, when we examine the behaviours of AE on 2D toy data sets  (\cref{fig:toy-bottleneck-2d}), we find that the identity mapping is not trivial to be learnt despite using AE with skip connections and very high latent dimensions. While this observation occurs on such a low dimensional data, this implies it could be more unlikely to learn the identity mapping for higher dimensional data due to higher degrees of freedom. This critical observation challenges the long-held belief that AEs must have bottlenecks, freeing the modeller from limiting to bottlenecked architectures.


% We illustrate the behaviours of AEs on 2D toy data sets and find that even with skip connections and very wide latent dimensions, the AE does not learn the identity mapping. 
\begin{figure}[hbtp]
\centerline{\includegraphics[width=\columnwidth]{images/2d-toy-bottleneck-infinite.png}}
\caption{\ExNLLShort using deterministic AE, BAE (anchored ensembling) and VAE with N($\hat{x}$,1) likelihood with/without skip connections on 2D toy data sets. Brighter (darker) region has lower (higher) \ExNLLShort values and log-scale of contour is used for higher visibility. The encoder architecture has fully connected layers with nodes of 2-50-50-50-dim(\textbf{z}) where dim(\textbf{z})=1 for undercomplete AE and dim(\textbf{z})=100 for overcomplete AE. We use SELU activation \cite{klambauer2017self} for every layer and sigmoid activation for the final layer. The darker contours away from the training points show that the deterministic AE, BAE and VAE do not learn the identity mapping despite being overparameterised and having skip connections.}
\label{fig:toy-bottleneck-2d}
\end{figure}

We suggest several reasons which prevent AEs from learning the identity mapping: high degree of non-linearity in the AE, the regularisation induced by modern deep learning optimisers (e.g. Adam \cite{kingma2014adam}) and by the priors over parameters. In this chapter, we provide empirical results to demonstrate that learning the identity mapping is non-trivial, despite removing the bottleneck; theoretical proofs are left for future work.

\section{Methods}
\subsection{Bayesian autoencoders}
Suppose we have a set of data $X^{train} = {\{\textbf{x}_1,\textbf{x}_2,\textbf{x}_3,...\textbf{x}_N\}}$, $\textbf{x}_{i} \in \rm I\!R^{D}$. An AE is an NN parameterised by $\theta$, and consists of two parts: an encoder $f_\text{encoder}$, for mapping input data $\textbf{x}$ to a latent embedding, and a decoder $f_\text{decoder}$ for mapping the latent embedding to a reconstructed signal of the input $\hat{\textbf{x}}$ (i.e. $\hat{\textbf{x}} = {f_{\theta}}(\textbf{x}) = f_\text{decoder}(f_\text{encoder}(\textbf{x}))$) \cite{goodfellow2016deep}. 

Bayes' rule can be applied to the parameters of the AE to create a BAE,
\begin{equation}\label{eq_posterior}
    p(\theta|X^{train}) = \frac{p(X^{train}|\theta)\, p(\theta)}{p(X^{train})} \\ ,
\end{equation}
where $p(X^{train}|\theta)$ is the likelihood and $p(\theta)$ is the prior distribution of the AE parameters. The log-likelihood for a diagonal Gaussian distribution is,
\begin{equation} \label{eq_gaussian_loss}
\log{p(\textbf{x}|\theta)} = -(\frac{1}{D} \sum^{D}_{i=1}{\frac{1}{2\sigma_i^2}}(x_i-\hat{x_i})^2 + \frac{1}{2}\log{\sigma_i^2})
\end{equation} 
where $\sigma_i^2$ is the variance of the Gaussian distribution. For simplicity, we use an isotropic Gaussian likelihood with $\sigma_i^2=1$ in this study, since the mean-squared error (MSE) function is proportional to the NLL. For brevity, we denote the NLL score $\minus\log{p(\textbf{x}|\theta)}$, as $\NLLfunc{\textbf{x})}$. For the prior distribution, we use an isotropic Gaussian prior which effectively leads to $L_2$ regularisation.

Since Equation~\ref{eq_posterior} is analytically intractable for a deep NN, various approximate methods have been developed such as Stochastic Gradient Markov Chain Monte Carlo (SGHMC) \cite{chen2014stochastic}, Monte Carlo Dropout (MCD) \cite{gal2016dropout}, Bayes by Backprop (BBB) \cite{blundell2015weight}, and anchored ensembling \cite{pearce2020uncertainty} to sample from the posterior distribution. In contrast, a deterministic AE has its parameters estimated using maximum likelihood estimation (MLE) or maximum a posteriori (MAP) when regularisation is introduced. The variational autoencoder (VAE) \cite{kingma2013auto} and BAE are AEs formulated differently within a probabilistic framework: in the VAE, only the latent embedding is stochastic while the $f_\text{encoder}$ and $f_\text{decoder}$ are deterministic and the model is trained using variational inference; on the other hand, the BAE, as an unsupervised BNN, has distributions over all parameters of $f_\text{encoder}$ and $f_\text{decoder}$. In short, the training phase of BAE entails using one of the sampling methods to obtain a set of approximate posterior samples $\{\hat{\theta}_m\}^M_{m=1}$. 

Then, during the prediction phase, we use the posterior samples to compute $M$ estimates of the NLL. The predictive density of a new datapoint $\mathbf{x}^*$ can be approximated as the mean of the posterior NLL estimates,
\begin{equation}
p(\textbf{x}^*| X^{train}) = \E{}_{\theta}[-\log{p(\textbf{x}^*|\theta)\,p(\theta|X^{train})}] \approx 
-\frac{1}{M}\sum^M_{m=1}p(\textbf{x}^*|\hat{\theta}_m)
\end{equation}

\subsection{Infinitely-wide BAE}
In the infinite-width limit, a BNN is equivalent to a Gaussian process with an NN kernel. In recent years, the results have been extended to modern architectures such as convolutional NNs, LSTM and transformers. We apply the NNGP to the AE, resulting in the infinitely-wide BAE, eliminating the bottleneck. 

Various benefits of NNGP exists: having a closed-form solution and the ability to model a BNN with infinitely many parameters. 

However, NNGP suffers from a computational complexity of $O(N^3)$, limiting its scalability to datasets with many training examples. Further, infinite NNs do not always outperform finite NNs; reasons for their underperformance remain an active area of research \cite{aitchison2020bigger, lee2020finite}. 

% Libraries such as NTK has simplified the conversion from a finite-BNN to an infinite-BNN.

% The extension of the NNGP derivation to existing architectures is an active area of research. 
% Having infinite parameters is of interest since NNs typically improve in performance with an increasing number of parameters.

\section{Experimental Setup}

We describe the datasets and models used in our experiments. The full code for reproducing results will be released upon the acceptance of this paper.

\subsection{Datasets}
Several types of data are included in our experiments. For image data, we train models on the FashionMNIST, treated as the inlier set, and test it against the MNIST as the anomalous set. We do the same for the pair CIFAR (inlier) vs SVHN (anomalous). For tabular data, we use 8 datasets from the ODDS collection: Cardio, Lympho, Optdigits, Ionosphere, Pendigits, Thyroid, Vowels and Pima.

For time-series data, we use the ZeMA and STRATH datasets, consisting of multiple sensors to detect anomalies in industrial settings. In the ZeMA dataset, the tasks are to detect anomalies in the subsystems of a hydraulic test rig. We consider the healthiest state of the subsystems as inliers and the rest as anomalies. While, in the STRATH dataset, the tasks are to detect defective parts manufactured from a radial forging facility; different sensors are used for each task (see \cref{table:des_zema_strath}). Geometric measurements of each forged part are available as target quality indicators.

We describe the data preprocessing as follows. For image datasets, we use the default split of train-test sets. For the ODDS, ZeMA and STRATH datasets, we split the inliers into train-test set of 70:30 ratio, and include anomalies in the test set. We apply min-max scaling with care to prevent train-test bias by fitting the scaler to the train set instead of the entire inlier set. For ZeMA, we downsample the pressure sensor to 1Hz and use the temperature data as provided; for STRATH, we downsample the data by tenfold and segment only the forging phase.  To label inliers and anomalies, we focus our analysis on the \textit{38 diameter@200} dimension of the forged parts. Anomalies are flagged by applying the Tukey's fences method \cite{tukey1977exploratory} on the absolute difference between the measured and nominal dimensions. 

\input{tables/description_zema_strath}

\subsection{Models}
We train variants of AEs: deterministic AE, VAE and BAE. For the BAE, we test several inference methods: MCD, BBB and anchored ensembling, always assuming an isotropic Gaussian prior over weights. The number of posterior samples is set to $M=100$ for the VAE, BAE-MCD and BAE-BBB, while $M=10$ for the BAE-Ensemble. We set a fixed learning rate of 0.001 for STRATH, while the learning rates for the other datasets are searched with a learning rate finder, employing a cyclic learning rate \cite{smith2017cyclical}. The Adam optimiser is used and the training epochs for FashionMNIST, CIFAR, ODDS, ZeMA and STRATH are 20, 20, 300, 100, 100, respectively. The weight decay is set to $1\times{10^{-11}}$ for FashionMNIST and CIFAR, and $1\times{10^{-10}}$ for ODDS, ZeMA and STRATH.

\input{tables/all_architecture}

The architectures of finite AEs are described in \cref{table:all-architecture}. Models in all datasets, except ZeMA, apply layer normalisation [] before the activation function. The size of latent dimensions is set to the flattened input dimensions multiplied by factors of $\times{\frac{1}{10}}, \times{\frac{1}{2}}, \times{1}$, including $\times{2}$ (for FashionMNIST and CIFAR) and $\times{10}$ (for ODDS, ZeMA and STRATH). For the infinite-width BAEs, we implement 7 dense layers (including the encoder and decoder) using an NNGP kernel on all datasets. The bias terms are turned off for dense and convolutional layers. Leaky relu [] is used for all intermediate layers while the sigmoid function [] is used for the final output layer.


\section{Results and discussion}
% tables 
% additional results?
% which datasets? ODDS, CIFAR, ZEMA+STRATH.
% infinite BAE + Normal BAEs

% the BAE models without bottleneck consistently achieve the best performances.
In Table XX, the AE models without bottleneck for many datasets, have achieved AUROC scores of $\ge0.8$, indicating that the identity function has not been learnt. This is true even for the infinitely-wide BAEs; they achieve the best performance on the ZEMA dataset.

The benefits of bottleneck removal are further quantified by the highest mean treatment effect achieved by either model types B, C or D. Notably, on CIFAR vs SVHN, type A models attain a poor mean AUROC score of 0.618, in contrast to type B and type D models with a mean AUROC score of $\ge0.8$.  Our results suggest that the poor OOD detection in extant works on AEs stems from the use of bottlenecked architectures. Nonetheless, the types of bottleneck removal scheme vary in performance for each dataset; we do not find a scheme which consistently outperforms other schemes. 

Switching from an AE to a BAE improves performance, as the best performing BAE achieves the highest AUROC score for all datasets. This gain is attributed to Bayesian model averaging \cite{hinne2020bma}, accounting for uncertainty in model parameters. In contrast, the VAE, which has only the latent layer probabilistic, does not perform as well as the BAE which probabilistic model accounts for all layers.

% ===


Many non-bottlenecked models have achieved AUROC scores $\ge{0.8}$, indicating improvements over the baseline performance, and that the identity function has not been learnt. We observe this even for the infinitely-wide BAEs, despite being overparameterised with infinite parameters. 

% POSSIBLE CITE (READ THIS): our result shows that increasing depth and width in neural networks leads to maps that are more contractive around training examples, thereby allowing for storage and retrieval of more training examples. == "Overparameterized neural networks implement associative memory"


% main points
1. Practitioners should not limit to only bottlenecked AEs, as non-bottlenecked models can potentially perform better. 
2. Further, using either one of the schemes of bottleneck removal can be better than the others.
3. The identity function is not as trivial to be learnt as previously assumed. 
4. While we lack theoretical proof that non-bottlenecked AEs never learn the identity function, the contrary is true; there is no proof, in previous works, that they will learn the identity function.
5. We do not argue that removing the bottleneck will \textit{always} improve the performance, since the best ML model for any task is data dependent due to no free lunch theorem [kevin murphy].

% limit discussion to on AD, not clustering or dimensinality reduction.

% change figure to say non-bottlenecked, instead of no bottleneck

% 4. From a probabilistic viewpoint, the BAE is a density estimation model. 
% on switching AE to BAE
3. Switching from a deterministic AE to a BAE improves performance.



% on infinite BAE
On average, infinitely-wide BAEs underperform their finite counterparts in our experiments. There are, nonetheless, several instances where the infinitely-wide BAEs outperform their finite counterparts. In light of their potential, future work should develop variants of infinitely-wide BAEs. Further, their closed-form solutions should facilitate theoretical work on understanding and proving the reasons for not learning the identity function. Possible directions include understanding the connection between BAEs as predictive density models and kernel density estimation.




% it is worthwhile for comparing against  


% It may not necessarily have learnt the identity function: the data complexity, amount of training examples and hyperparameters may play an influencing role. 

% in which the importance of handling uncertainty model parameters grow with the number of model parameters

\section{Related work}
% Skip connections (vs COLLIN)
Several works have explored the use of skip connections in AEs for image denoising \cite{zhao2018,mao2016} and audio separation \cite{liu2018} tasks. Closest to our work is \cite{collin2021, kim2021} which modelled AEs with skip connections for image anomaly detection but our work differs in several ways. First, we attempt to shed light on a broader issue of whether AEs need bottlenecks at all by suggesting the identity mapping is not trivial to be learnt by AEs. Additionally, we compare against overparameterised AEs and visualise their behaviours on toy data set. Second, we find that even without the denoising scheme, AEs with skip connections are unable to learn the identity mapping and may still perform well for anomaly detection. However, note that we do not claim that skip AEs are always better as there are instances where non-skip AEs exhibit better performances which dependent on the data set. Third, we include comparisons between deterministic AEs, VAEs and BAEs trained under different approximate sampling methods and cast light on BAE as a density estimation model. Fourth, our study extends the use of skip AEs from image data to multisensors data. 



\section{Conclusion}
Visualised on low dimensional toy data, we found the identity mapping is not trivial to be learnt even when the AE does not have a bottleneck architecture. We extended the experiments to STRATH data set in which we confirm that AEs without bottleneck may still perform well. Note that we focused on anomaly detection and our result is not applicable to other use cases of AEs, e.g. dimensionality reduction and clustering, in which a bottleneck may prove essential.


% TODO:
% Get base from the STRATH report
% All datasets: +ODDS datasets 
% results and discussion 
% related work
% experiment setup
% Connection to GP: Infinite BAE

% methods, experiment setup, conclusion

% OTHERS:
% Wrap into a conference paper?
% extend LL discussions to manufacturing DT

% \input{tables/FashionMNIST_bottleneck}
% \input{tables/CIFAR_bottleneck}
% \input{tables/ZEMA_bottleneck}
\input{tables/bottleneck_full}

\begin{figure}[hbtp]
\centerline{\includegraphics[width=\columnwidth]{images/bottleneck_boxplot_ens.png}}
\caption{\ExNLLShort using deterministic AE, BAE (anchored ensembling) and VAE with N($\hat{x}$,1) likelihood with/without skip connections on 2D toy data sets. Brighter (darker) region has lower (higher) \ExNLLShort values and log-scale of contour is used for higher visibility. The encoder architecture has fully connected layers with nodes of 2-50-50-50-dim(\textbf{z}) where dim(\textbf{z})=1 for undercomplete AE and dim(\textbf{z})=100 for overcomplete AE. We use SELU activation \cite{klambauer2017self} for every layer and sigmoid activation for the final layer. The darker contours away from the training points show that the deterministic AE, BAE and VAE do not learn the identity mapping despite being overparameterised and having skip connections.}
\label{fig:toy-bottleneck-2d}
\end{figure}

% We stress that extant works on AEs have not reported success in OOD detection for CIFAR vs SVHN, in which our results suggest that it is due to the use of bottlenecked architectures. 
% \Infbae % While it is possible for bottlenecked models to outperform those without bottleneck for some datasets, 
% we posit the optimal architecture and model capacity is dataset dependent.
% \textbf{Effect of removing bottleneck.} In \cref{fig:need-for-bottleneck}, none of the models exhibited AUROC $\leq{0.6}$ despite not having any bottleneck by increasing the latent dimensions and/or adding skip connections. This implies the identity mapping was not learnt by any of the AEs even on a higher dimensional data. Furthermore, we notice a positive effect as we increase the latent dimensions of the skip VAE for L-ACTpos sensor (\cref{fig:need-for-bottleneck}(a)) and shows that having a wide latent dimension is not always detrimental for anomaly detection.      

% Having skip connections bring about a significant change to the AE’s performance. Although this effect has been positive for (b) and (c), it is not the case for (a). Contrary to \cite{collin2021,kim2021}, this shows that adding skip connection may not always be a good addition to the AE as it may depend on the input data\footnote{In the STRATH data set, this refers to the chosen combination of sensors and preprocessing steps.}. The primary implication of this finding is that practitioners do not need to enforce a bottleneck in AEs for anomaly detection and that a wider architecture search could be employed when optimising for performance.

% does not need dropout layers.

==> depracated/body_20220124.tex <==
% TODO:
% Get base from the STRATH report
% All datasets: +ODDS datasets 
% results and discussion 
% related work
% experiment setup
% Connection to GP: Infinite BAE

% === MAIN POINTS ===
% 1. Practitioners should not limit to only bottlenecked AEs, as non-bottlenecked models can potentially perform better. 
% 2. Further, using either one of the schemes of bottleneck removal can be better than the others.
% 3. The identity function is not as trivial to be learnt as previously assumed. 
% 4. While we lack theoretical proof that non-bottlenecked AEs never learn the identity function, the contrary is true; there is no proof, in previous works, that they will learn the identity function.
% 5. We do not argue that removing the bottleneck will \textit{always} improve the performance, since the best ML model for any task is data dependent due to no free lunch theorem [kevin murphy].
% limit discussion to on AD, not clustering or dimensinality reduction.
% change figure to say non-bottlenecked, instead of no bottleneck
% \section{Do AEs need a bottleneck?}

% with skip connections and very high latent dimensions
% This critical observation challenges the long-held belief that AEs must have bottlenecks, freeing the modeller from limiting to bottlenecked architectures.
%  is not as trivial to be learnt by modern AE architectures as previously assumed.
% Pushing our experiments further, we are the first to experiment with infinitely-wide BAEs for anomaly detection; surprisingly, they demonstrate improvements over the baseline AEs, despite strongly opposing the conventional use of bottlenecked architectures.
% The results are from extensive experiments, covering various types of data for anomaly detection and probabilistic variants of the AEs: variational autoencoder and Bayesian autoencoders.
% Nonetheless, the use of skip connections in AE is not common for anomaly detection as it is assumed to promote learning the identity mapping.
% [put a picture here]
% Our work differs by finding that even without the denoising scheme, AEs with skip connections are unable to learn the identity function and may still perform well for anomaly detection. Moreover, our work attempts to shed light on a broader issue of whether AEs need bottlenecks at all.
% We illustrate the behaviours of AEs on 2D toy data sets and find that even with skip connections and very wide latent dimensions, the AE does not learn the identity mapping. 
% Motivated by this observation, we therefore question the mandatory use of bottlenecked AEs for anomaly detection. Our extensive experiments on various types of data and AEs (deterministic AEs, variational autoencoders and Bayesian autoencoders) demonstrate the effective use of non-bottlenecked architectures, demonstrating the difficulty of learning the identity function. Further, we are the first to experiment with infinitely-wide AEs for anomaly detection; unexpectedly, they yield improvements over the baseline, despite having infinite parameters and strongly opposing the conventional use of bottlenecked architectures. 

% While we lack theoretical proof that non-bottlenecked AEs will never learn the identity function, the contrary is true; there is no proof, to this date, that they will learn the identity function.

\section{Introduction}

Numerous works have demonstrated the successful use of autoencoders (AEs), a type of unsupervised neural network (NN), for anomaly detection \cite{pang2021}. AEs are optimised to reconstruct a set of training data with minimal error. When given anomalous data with high dissimilarity from the training data, the AEs reconstruct them with high error. Therefore, the reconstruction error is a measure of data anomalousness; by placing a threshold, we can effectively classify data points as inliers or anomalies.

Extant works claim that AEs will trivially learn the identity function when no constraints are placed \cite{ruff2018, ng2011sparse}. If this were to occur, AEs will perfectly reconstruct any inputs (regardless whether it is anomalous or not), and hence the reconstruction loss will be low for all inputs, leading to unreliable anomaly detection. To prevent this, it is common to impose a bottleneck in the architecture, resulting in an undercomplete architecture: the output of the encoder has much lower dimensions than the input. However, most works describe the need for a bottleneck analogically and report only the empirical performance of bottlenecked AEs, without comparing them against non-bottlenecked AEs \cite{chen2018autoencoder, chow2020, kim2020, mujeeb2019, ruff2018}. 

\textbf{Why should we care about non-bottlenecked AEs?} By limiting to bottlenecked architectures, we miss the potential of achieving better performance with non-bottlenecked AEs. Therefore, in this work, we study the use of non-bottlenecked AEs for anomaly detection. We investigate various ways of removing the bottleneck, including expanding the latent dimensions and introducing skip connections. We further propose the infinitely-wide AE as an extreme example. Extensive experiments demonstrate the empirical success of non-bottlenecked AEs in detecting anomalies over bottlenecked AEs, indicating the former have failed to learn the identity function, contrary to conventional belief.

In light of this, we suggest that rethinking about AEs is needed. We adopt the probabilistic formulation of Bayesian autoencoders (BAEs), viewing them as density estimation models that benefit from having higher expressivity. The Bayesian framework also provides a sound foundation for theoretical analysis of our findings in future work.

\section{Methods}

\subsection{Bayesian autoencoders}
Suppose we have a set of data $X^{train} = {\{\textbf{x}_1,\textbf{x}_2,\textbf{x}_3,...\textbf{x}_N\}}$, $\textbf{x}_{i} \in \rm I\!R^{D}$. An AE is an NN parameterised by $\theta$, and consists of two parts: an encoder $f_\text{encoder}$, for mapping input data $\textbf{x}$ to a latent embedding, and a decoder $f_\text{decoder}$ for mapping the latent embedding to a reconstructed signal of the input $\hat{\textbf{x}}$ (i.e. $\hat{\textbf{x}} = {f_{\theta}}(\textbf{x}) = f_\text{decoder}(f_\text{encoder}(\textbf{x}))$) \cite{goodfellow2016deep}. 

Bayes' rule can be applied to the parameters of the AE to create a BAE,
\begin{equation}\label{eq_posterior}
    p(\theta|X^{train}) = \frac{p(X^{train}|\theta)\, p(\theta)}{p(X^{train})} \\ ,
\end{equation}
where $p(X^{train}|\theta)$ is the likelihood and $p(\theta)$ is the prior distribution of the AE parameters. The log-likelihood for a diagonal Gaussian distribution is,
\begin{equation} \label{eq_gaussian_loss}
\log{p(\textbf{x}|\theta)} = -(\frac{1}{D} \sum^{D}_{i=1}{\frac{1}{2\sigma_i^2}}(x_i-\hat{x_i})^2 + \frac{1}{2}\log{\sigma_i^2})
\end{equation} 
where $\sigma_i^2$ is the variance of the Gaussian distribution. For simplicity, we use an isotropic Gaussian likelihood with $\sigma_i^2=1$ in this study, since the mean-squared error (MSE) function is proportional to the NLL. For brevity, we denote the NLL score $\minus\log{p(\textbf{x}|\theta)}$, as $\NLLfunc{\textbf{x})}$. For the prior distribution, we use an isotropic Gaussian prior which effectively leads to $L_2$ regularisation.

Since Equation~\ref{eq_posterior} is analytically intractable for a deep NN, various approximate methods have been developed such as Stochastic Gradient Markov Chain Monte Carlo (SGHMC) \cite{chen2014stochastic}, Monte Carlo Dropout (MCD) \cite{gal2016dropout}, Bayes by Backprop (BBB) \cite{blundell2015weight}, and anchored ensembling \cite{pearce2020uncertainty} to sample from the posterior distribution. In contrast, a deterministic AE has its parameters estimated using maximum likelihood estimation (MLE) or maximum a posteriori (MAP) when regularisation is introduced. The variational autoencoder (VAE) \cite{kingma2013auto} and BAE are AEs formulated differently within a probabilistic framework: in the VAE, only the latent embedding is stochastic while the $f_\text{encoder}$ and $f_\text{decoder}$ are deterministic and the model is trained using variational inference; on the other hand, the BAE, as an unsupervised BNN, has distributions over all parameters of $f_\text{encoder}$ and $f_\text{decoder}$. In short, the training phase of BAE entails using one of the sampling methods to obtain a set of approximate posterior samples $\{\hat{\theta}_m\}^M_{m=1}$. 

Then, during the prediction phase, we use the posterior samples to compute $M$ estimates of the NLL. The predictive density of a new datapoint $\mathbf{x}^*$ can be approximated as the mean of the posterior NLL estimates,
\begin{equation}
p(\textbf{x}^*| X^{train}) = \E{}_{\theta}[-\log{p(\textbf{x}^*|\theta)\,p(\theta|X^{train})}] \approx 
-\frac{1}{M}\sum^M_{m=1}p(\textbf{x}^*|\hat{\theta}_m)
\end{equation}

% BAE as density estimation model
The Bayesian formulation allows us to view AEs as regularised probability density estimators. BAEs model the training data distribution, assigning lower density scores to data with higher dissimilarity from the majority of training data. It is not unconventional for density estimators to have infinite parameters; they can model an arbitrary distribution well with high expressivity \cite{chen2006probability, sriperumbudur2017density}. 

% Therefore, we propose the BAE with infinite parameters in the following section.
% having more parameters and capacity may help in modelling the training data. 
% with automatic regularisation. 
% Further, it is not unusual for density estimators to benefit from infinite parameters with high expressivity. 
\subsection{How to remove the bottleneck?}
A bottleneck is implemented when the latent dimensions are smaller than the input dimensions $\text{dim}(f_\text{encoder}(\textbf{x}))<\text{dim}(\textbf{x})$ and there is no way for intermediate outputs of the encoder to bypass this bottleneck layer. Therefore, we can eliminate the bottleneck using either or both of the following methods: (1) simply expand the size of the latent dimensions to be equal to or greater than the flattened input dimensions, also known as an overcomplete architecture, and (2) introduce long-range skip connections from the encoder to the decoder akin to a U-Net architecture \cite{unet2015}, thereby allowing each layer's data flow to bypass the bottleneck. We tabulate architectures which are and are not bottlenecked in Table XX. 

\begin{table}[hbtp]
\centering
    \begin{tabular}{ccc}
    \hline
    Architecture type & Latent dimensions & Skip connections \\ \hline
    \textbf{With bottleneck} &  &  \\
    A & Undercomplete & \xmark \\ \hline
    \textbf{Without bottleneck} &  &  \\
    B & Undercomplete & \cmark \\
    C & Overcomplete & \xmark \\
    D & Overcomplete & \cmark \\ \hline
    \end{tabular}
\end{table}
% why skip connections?
\textbf{Why skip connections?} Skip connections allow better flow of information in NNs with many layers, leading to a smoother loss landscape \cite{li2017visualizing} and easier optimisation without additional computational complexity \cite{he2016deep}. Recently, \cite{collin2021, kim2021} reported that AEs with skip connections outperform those without on image anomaly detection. A concern with implementing skip connections, however, is that it may contribute to learning the identity function. In preventing this, \cite{collin2021} trained the skip-AEs to output clean images out of noisy images (also known as denoising AEs). 
In our work, we do not implement denoising AEs and further, [] shown it was...
% explicitly attempt 


% One challenge of modelling such denoising AEs for anomaly detection is the choice of synthetic corruption method, also known as data augmentation, which largely depends on the type of data (e.g. image, tabular, time-series, etc.) and type of expected anomalies (e.g. stained images) making it not easily generalisable to other data types.  

\subsection{Infinitely-wide BAE}
In the infinite-width limit, a BNN is equivalent to a Gaussian process with an NN kernel. In recent years, the results have been extended to modern architectures such as convolutional NNs, LSTM and transformers. We propose extending the NNGP to the AE, resulting in the infinitely-wide BAE with a non-bottlenecked architecture.  

Various benefits of NNGP exist: having a closed-form solution and modelling a BNN with infinitely many parameters. The first promotes a theoretical understanding of the BNN's behaviour and instil trust in their adoption by increasing algorithmic transparency []. Secondly, since modern NNs succeed over traditional ML models by increasing the number of parameters, it is interesting to know how well they perform with infinite parameters []. However, NNGP suffers from a computational complexity of $O(N^3)$, limiting its scalability to datasets with many training examples. In addition, infinite NNs do not always outperform finite NNs; reasons for their underperformance remain an active area of research \cite{aitchison2020bigger, lee2020finite}. 

\subsection{Evaluating the identity function}

The identity function is successfully learnt when $f_{\theta}(\textbf{x}) = \textbf{x}$ holds true for all \textbf{x} and therefore the reconstruction loss or NLL is always 0, rendering it useless for distinguishing inliers from anomalies.   

Surprisingly, when we examine the behaviours of AE on 2D toy data sets  (\cref{fig:toy-bottleneck-2d}), we find that the identity mapping is not trivial to be learnt despite using various types of non-bottlenecked AEs. Consequently, this observation on low-dimensional data implies it is more unlikely to learn the identity mapping on high-dimensional data due to higher degrees of freedom. 

\begin{figure}[hbtp]
\centerline{\includegraphics[width=\columnwidth]{images/2d-toy-bottleneck-infinite.png}}
\caption{\ExNLLShort using deterministic AE, BAE (anchored ensembling) and VAE with N($\hat{x}$,1) likelihood with/without skip connections on 2D toy data sets. Brighter (darker) region has lower (higher) \ExNLLShort values and log-scale of contour is used for higher visibility. The encoder architecture has fully connected layers with nodes of 2-50-50-50-dim(\textbf{z}) where dim(\textbf{z})=1 for undercomplete AE and dim(\textbf{z})=100 for overcomplete AE. We use SELU activation \cite{klambauer2017self} for every layer and sigmoid activation for the final layer. The darker contours away from the training points show that the deterministic AE, BAE and VAE do not learn the identity mapping despite being overparameterised and having skip connections.}
\label{fig:toy-bottleneck-2d}
\end{figure}

We suggest several reasons preventing the AEs from learning the identity mapping: high degree of non-linearity in the AE, the regularisation induced by modern deep learning optimisers (e.g. Adam \cite{kingma2014adam}) and by the priors over parameters. In this chapter, we provide empirical results to demonstrate that learning the identity mapping is non-trivial, despite removing the bottleneck; theoretical proofs are left for future work.

% Libraries such as NTK has simplified the conversion from a finite-BNN to an infinite-BNN.
% The extension of the NNGP derivation to existing architectures is an active area of research. 
% Having infinite parameters is of interest since NNs typically improve in performance with an increasing number of parameters.

\section{Experimental Setup}

We describe the datasets and models used in our experiments. The full code for reproducing results will be released upon the acceptance of this paper.

\subsection{Datasets}
Several types of data are included in our experiments. For all datasets, we train our models on the inliers training set and during testing, we compute AUROC scores on the test set consisting of inliers and anomalies. For image data, we use two pairs of unrelated datasets (inliers vs anomalies) commonly used in previous works: FashionMNIST vs MNIST, and CIFAR vs SVHN. For tabular data, we use 8 datasets from the ODDS collection: Cardio, Lympho, Optdigits, Ionosphere, Pendigits, Thyroid, Vowels and Pima. For time-series data, we use the ZeMA and STRATH datasets, consisting of multiple sensors to detect anomalies in industrial settings. 

In the ZeMA dataset, the tasks are to detect deterioration in the subsystems of a hydraulic test rig. We consider the data from the healthiest state of the subsystems as inliers and the rest as anomalies. While, in the STRATH dataset, different sensors are used in each task (see \cref{table:des_zema_strath}) to detect defective parts manufactured from a radial forging process consisting of heating and forging phases. Geometric measurements of each forged part are available as target quality indicators. To label inliers and anomalies, we focus our analysis on the \textit{38 diameter@200} of the forged parts. Anomalies are flagged by applying the Tukey's fences method \cite{tukey1977exploratory} on the absolute difference between the measured and nominal dimensions. 

\subsection{Preprocessing}
For image datasets, we use the default split of train-test sets and rescale pixel values to [0,1]. For the ODDS, ZeMA and STRATH datasets, we split the inliers into train-test sets of 70:30 ratio, and include all anomalies in the test set. We apply min-max scaling with care to prevent train-test bias by fitting the scaler to the train set instead of the entire inlier set. For ZeMA, we downsample the pressure sensor to 1Hz and use the temperature data as provided; for STRATH, we downsample the data by tenfold and segment only the forging phase.  

\input{tables/description_zema_strath}

\subsection{Models}
We train variants of AEs: deterministic AE, VAE, and BAEs with several inference methods: MCD, BBB and anchored ensembling. All models use isotropic Gaussian priors over weights. The number of posterior samples is set to $M=100$ for the VAE, BAE-MCD and BAE-BBB, while $M=10$ for the BAE-Ensemble. We set a fixed learning rate of 0.001 for STRATH, while the learning rates for the other datasets are searched with a learning rate finder, employing a cyclic learning rate \cite{smith2017cyclical}. The Adam optimiser is used and the training epochs for FashionMNIST, CIFAR, ODDS, ZeMA and STRATH are 20, 20, 300, 100, 100, respectively. The weight decay is set to $1\times{10^{-11}}$ for FashionMNIST and CIFAR, and $1\times{10^{-10}}$ for ODDS, ZeMA and STRATH.

\input{tables/all_architecture}

The architectures of finite AEs are described in \cref{table:all-architecture}. Models in all datasets, except ZeMA, apply layer normalisation [] before the activation function. The size of latent dimensions is set to the flattened input dimensions multiplied by factors of $\times{\frac{1}{10}}, \times{\frac{1}{2}}, \times{1}$, including $\times{2}$ (for FashionMNIST and CIFAR) and $\times{10}$ (for ODDS, ZeMA and STRATH). For the infinite BAEs, we implement 7 infinitely-wide dense layers (including the encoder and decoder) using an NNGP kernel on all datasets. The bias terms are turned off for dense and convolutional layers. Leaky relu [] is used for all intermediate layers while the sigmoid function [] is used for the final output layer.


\section{Results and discussion}
% tables 
% additional results?
% which datasets? ODDS, CIFAR, ZEMA+STRATH.
% infinite BAE + Normal BAEs

% the BAE models without bottleneck consistently achieve the best performances.
% In Table XX, the AE models without bottleneck for many datasets, have achieved AUROC scores of $\ge0.8$, indicating that the identity function has not been learnt. This is true even for the infinitely-wide BAEs; they achieve the best performance on the ZEMA dataset.

% The benefits of bottleneck removal are further quantified by the highest mean treatment effect achieved by either model types B, C or D. Notably, on CIFAR vs SVHN, type A models attain a poor mean AUROC score of 0.618, in contrast to type B and type D models with a mean AUROC score of $\ge0.8$.  Our results suggest that the poor OOD detection in extant works on AEs stems from the use of bottlenecked architectures. Nonetheless, the types of bottleneck removal scheme vary in performance for each dataset; we do not find a scheme which consistently outperforms other schemes. 

% Switching from an AE to a BAE improves performance, as the best performing BAE achieves the highest AUROC score for all datasets. This gain is attributed to Bayesian model averaging \cite{hinne2020bma}, accounting for uncertainty in model parameters. In contrast, the VAE, which has only the latent layer probabilistic, does not perform as well as the BAE which probabilistic model accounts for all layers.

% ===


% Many non-bottlenecked models have achieved AUROC scores $\ge{0.8}$, indicating improvements over the baseline performance, and that the identity function has not been learnt. We observe this even for the infinitely-wide BAEs, despite being overparameterised with infinite parameters. 

% POSSIBLE CITE (READ THIS): our result shows that increasing depth and width in neural networks leads to maps that are more contractive around training examples, thereby allowing for storage and retrieval of more training examples. == "Overparameterized neural networks implement associative memory"

% =======================

% 4. From a probabilistic viewpoint, the BAE is a density estimation model. 
% on switching AE to BAE
% 3. Switching from a deterministic AE to a BAE improves performance.

% =====
% The performance of bottleneck removal schemes varies for each dataset; we do not find a scheme which consistently outperforms other schemes. 

% discuss table of performance, bt vs non-bt

% A vs BCD
Many non-bottlenecked models (type B, C and D) have performed above the baseline with mean AUROC scores $\ge{0.8}$, indicating the identity function has not been learnt. Also, their positive average treatment effects (ATE) indicate improvements over the bottlenecked models (type A). In addition, on most datasets, the best mean AUROC scores have been achieved by one of the non-bottlenecked models, except on FashionMNIST vs MNIST, which has the bottlenecked model (BAE-BBB, type A), marginally beating the second-best model (BAE-BBB, type C) by 0.1 AUROC.

% CIFAR vs SVHN
Focusing on CIFAR vs SVHN, our results provide new insight into previous works which reported poor performance on AEs. Notably, the best non-bottlenecked model (type B BAE-Ensemble, AUROC=$0.849$) and the \Infbae (AUROC=$0.771$) outperform the best bottlenecked model (type A BAE-Ensemble, AUROC=$0.696$). These results imply the poor performance could be fixed if previous works have explored on non-bottlenecked architectures.

% AE vs BAE
Switching from an AE to a BAE improves performance. The best performing BAEs achieve the highest AUROC scores on all datasets. The performance gain is attributed to Bayesian model averaging \cite{hinne2020bma}, accounting for uncertainty in model parameters. The best BAEs also outperform the VAEs, evidencing the advantage of addressing uncertainty over parameters of the entire model instead of the latent layer only.

%  On infinite-BAE
The \Infbae\, has performed better than random guessing with $\ge{0.7}$ AUROC on all datasets, indicating its inability of learning the identity function despite being infinitely parameterised. Although it does not score the highest mean AUROC, on a positive note, there are specific tasks on which the \Infbae\ outperforms other models with the highest median (e.g. see \cref{fig:boxplots-bottleneck} on Cardio, Thyroid, Pendigits and ZeMA(iii)). Additionally, the deterministic computation of the \Infbae\ contributes to the lower variability in performance for these tasks, signifying its robustness. 



% it is worthwhile for comparing against  


% It may not necessarily have learnt the identity function: the data complexity, amount of training examples and hyperparameters may play an influencing role. 

% in which the importance of handling uncertainty model parameters grow with the number of model parameters

\section{Related work}
% Skip connections (vs COLLIN)

% Several works have explored the use of skip connections in AEs for image denoising \cite{zhao2018,mao2016} and audio separation \cite{liu2018} tasks. 

Closest to our work is \cite{collin2021, kim2021} which modelled AEs with skip connections for image anomaly detection but our work differs in several ways. First, we attempt to shed light on a broader issue of whether AEs need bottlenecks at all by suggesting the identity mapping is not trivial to be learnt by AEs. Additionally, we compare against overparameterised AEs and visualise their behaviours on toy data set. Second, we find that even without the denoising scheme, AEs with skip connections are unable to learn the identity mapping and may still perform well for anomaly detection. However, note that we do not claim that skip AEs are always better as there are instances where non-skip AEs exhibit better performances which dependent on the data set. Third, we include comparisons between deterministic AEs, VAEs and BAEs trained under different approximate sampling methods and cast light on BAE as a density estimation model. Fourth, our study extends the use of skip AEs from image data to multisensors data. 



\section{Conclusion}
Visualised on low dimensional toy data, we found the identity mapping is not trivial to be learnt even when the AE does not have a bottleneck architecture. We extended the experiments to STRATH data set in which we confirm that AEs without bottleneck may still perform well. Note that we focused on anomaly detection and our result is not applicable to other use cases of AEs, e.g. dimensionality reduction and clustering, in which a bottleneck may prove essential.

In light of the potential, future work should develop variants of \Infbae. Their closed-form solutions can facilitate theoretical work on understanding and proving the reasons for not learning the identity function. Possible directions include understanding the connection between BAEs as predictive density models and kernel density estimation [].



% TODO:
% Get base from the STRATH report
% All datasets: +ODDS datasets 
% results and discussion 
% related work
% experiment setup
% Connection to GP: Infinite BAE

% methods, experiment setup, conclusion

% OTHERS:
% Wrap into a conference paper?
% extend LL discussions to manufacturing DT

% \input{tables/FashionMNIST_bottleneck}
% \input{tables/CIFAR_bottleneck}
% \input{tables/ZEMA_bottleneck}
\input{tables/bottleneck_full}

\begin{figure}[hbtp]
\centerline{\includegraphics[width=\columnwidth]{images/bottleneck_boxplot_ens.png}}
\caption{\ExNLLShort using deterministic AE, BAE (anchored ensembling) and VAE with N($\hat{x}$,1) likelihood with/without skip connections on 2D toy data sets. Brighter (darker) region has lower (higher) \ExNLLShort values and log-scale of contour is used for higher visibility. The encoder architecture has fully connected layers with nodes of 2-50-50-50-dim(\textbf{z}) where dim(\textbf{z})=1 for undercomplete AE and dim(\textbf{z})=100 for overcomplete AE. We use SELU activation \cite{klambauer2017self} for every layer and sigmoid activation for the final layer. The darker contours away from the training points show that the deterministic AE, BAE and VAE do not learn the identity mapping despite being overparameterised and having skip connections.}
\label{fig:boxplots-bottleneck}
\end{figure}

% We stress that extant works on AEs have not reported success in OOD detection for CIFAR vs SVHN, in which our results suggest that it is due to the use of bottlenecked architectures. 
% \Infbae % While it is possible for bottlenecked models to outperform those without bottleneck for some datasets, 
% we posit the optimal architecture and model capacity is dataset dependent.
% \textbf{Effect of removing bottleneck.} In \cref{fig:need-for-bottleneck}, none of the models exhibited AUROC $\leq{0.6}$ despite not having any bottleneck by increasing the latent dimensions and/or adding skip connections. This implies the identity mapping was not learnt by any of the AEs even on a higher dimensional data. Furthermore, we notice a positive effect as we increase the latent dimensions of the skip VAE for L-ACTpos sensor (\cref{fig:need-for-bottleneck}(a)) and shows that having a wide latent dimension is not always detrimental for anomaly detection.      

% Having skip connections bring about a significant change to the AE’s performance. Although this effect has been positive for (b) and (c), it is not the case for (a). Contrary to \cite{collin2021,kim2021}, this shows that adding skip connection may not always be a good addition to the AE as it may depend on the input data\footnote{In the STRATH data set, this refers to the chosen combination of sensors and preprocessing steps.}. The primary implication of this finding is that practitioners do not need to enforce a bottleneck in AEs for anomaly detection and that a wider architecture search could be employed when optimising for performance.

% does not need dropout layers.

==> tables/CIFAR10_table.tex <==
\begin{table}[H]
\caption{(CIFAR10 vs SVHN) AUROC for various models and likelihoods. Results where AUROC\textgreater{0.6} are in bold.}
\label{table-results-CIFAR10}
\resizebox{.65\textwidth}{!}{
\begin{tabular}{@{}llcccc@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Model}} & \multicolumn{1}{c}{\multirow{2}{*}{Likelihood}} & \multicolumn{4}{c}{AUROC}                                  \\ \cmidrule(l){3-6} 
\multicolumn{1}{c}{}                       & \multicolumn{1}{c}{}                            & $\mathrm{Var}_\theta(\hat{\textbf{x}}^*)$ & $\E_{\theta}\mathrm{(LL)}$ & $\mathrm{Var_{\theta}(LL)}$ & WAIC \\ \midrule
Deterministic AE                                         & Ber($\hat{x}^*$)                                             & -                & \textbf{0.601}       & -           & -           \\
Deterministic AE                                         & C-Ber($\hat{x}^*$)                                          & -                & \textbf{0.607}       & -           & -           \\
Deterministic AE                                         & N($\hat{x}^*$,1)                                               & -                & 0.038       & -           & -           \\ \midrule
VAE                                        & Ber($\hat{x}^*$)                                             & 0.492            & \textbf{0.604}       & 0.051       & \textbf{0.604}       \\
VAE                                        & C-Ber($\hat{x}^*$)                                           & 0.518            & \textbf{0.609}       & 0.077       & \textbf{0.609}       \\
VAE                                        & N($\hat{x}^*$,1)                                               & 0.522            & 0.045       & 0.048       & 0.045       \\ \midrule
BAE, MC-Dropout                            & Ber($\hat{x}^*$)                                             & 0.241            & \textbf{0.600}       & 0.113       & 0.599       \\
BAE, MC-Dropout                            & C-Ber($\hat{x}^*$)                                           & 0.214            & \textbf{0.607}       & 0.144       & \textbf{0.605}       \\
BAE, MC-Dropout                            & N($\hat{x}^*$,1)                                               & 0.260            & 0.051       & 0.088       & 0.051       \\ \midrule
BAE, BayesBB                                    & Ber($\hat{x}^*$)                                             & 0.377            & 0.572       & 0.211       & 0.570       \\
BAE, BayesBB                                    & C-Ber($\hat{x}^*$)                                           & 0.385            & 0.591       & 0.193       & 0.586       \\
BAE, BayesBB                                    & N($\hat{x}^*$,1)                                               & 0.359            & 0.094       & 0.131       & 0.094       \\ \midrule
BAE, Ensemble                              & Ber($\hat{x}^*$)                                             & 0.186            & \textbf{0.603}       & 0.086       & \textbf{0.603}       \\
BAE, Ensemble                              & C-Ber($\hat{x}^*$)                                           & 0.175            & \textbf{0.609}       & 0.104       & \textbf{0.609}       \\
BAE, Ensemble                              & N($\hat{x}^*$,1)                                               & 0.151            & 0.039       & 0.065       & 0.039       \\ \bottomrule
\end{tabular}
}
\end{table}


==> tables/CIFAR_bottleneck.tex <==
\begin{table}[H] 
\caption{AUROC scores for deterministic AE, VAE and BAE-Ensemble with various architectures (type A, B, C or D) are categorised as either with a bottleneck or without. For each dataset, the model scoring the highest AUROC is bolded.}
    % \begin{subtable}[h]{\textwidth}
    %     \centering
    %     \scriptsize \caption{ZEMA}
    %         \resizebox{0.8\textwidth}{!}{
    %             \begin{tabular}{@{}lcccc@{}}
    %             \toprule
    %              & ---Bottleneck--- & \multicolumn{3}{c}{------------------Without Bottleneck------------------} \\ 
    %              \multicolumn{1}{c}{Model} & \begin{tabular}[c]{@{}c@{}}A\\ Undercomplete\\ No skip\end{tabular} & \begin{tabular}[c]{@{}c@{}}B\\ Undercomplete\\ + skip\end{tabular} & \begin{tabular}[c]{@{}c@{}}C\\ Overcomplete\\ No skip\end{tabular} & \begin{tabular}[c]{@{}c@{}}D\\ Overcomplete\\ + skip\end{tabular} \\ \midrule

    %             % \multicolumn{1}{c}{Model} & \begin{tabular}[c]{@{}c@{}}A\\ Undercomplete\\ No skip\end{tabular} & \begin{tabular}[c]{@{}c@{}}B\\ Undercomplete\\ +skip\end{tabular} & \begin{tabular}[c]{@{}c@{}}C\\ Overcomplete\\ No skip\end{tabular} & \begin{tabular}[c]{@{}c@{}}D\\ Overcomplete\\ +skip\end{tabular} \\ \midrule

    %             Deterministic AE & 0.906 & 0.943 & 0.925 & 0.947 \\
    %             VAE & 0.895 & 0.938 & 0.892 & 0.947 \\
    %             BAE-MCD & 0.901 & 0.937 & 0.898 & 0.942 \\
    %             BAE-BBB & 0.900 & 0.947 & 0.907 & 0.936 \\ 
    %             BAE-Ensemble & 0.944 & 0.964 & 0.929 & 0.965 \\ 
    %             BAE-\scalebox{1.25}{$\infty$}  & - & - & 0.968 & \textbf{0.992} \\ \midrule
    %             \textbf{Mean} & 0.909 & 0.946 & 0.920 & 0.955 \\ \bottomrule
    %             \end{tabular}
    %         }
       
    % \end{subtable}
    % \hfill
    \begin{subtable}[h]{\textwidth}
        \centering
        \vskip 0.2in
        \scriptsize \caption{CIFAR vs SVHN}
            \resizebox{0.8\textwidth}{!}{
                \begin{tabular}{@{}lcccc@{}}
                \toprule
                 & ---Bottleneck--- & \multicolumn{3}{c}{------------------Without Bottleneck------------------} \\ 
                 \multicolumn{1}{c}{Model} & \begin{tabular}[c]{@{}c@{}}A\\ Undercomplete\\ No skip\end{tabular} & \begin{tabular}[c]{@{}c@{}}B\\ Undercomplete\\ + skip\end{tabular} & \begin{tabular}[c]{@{}c@{}}C\\ Overcomplete\\ No skip\end{tabular} & \begin{tabular}[c]{@{}c@{}}D\\ Overcomplete\\ + skip\end{tabular} \\ \midrule

                Deterministic AE & 0.686 & 0.833 & 0.660 & 0.815 \\
                VAE & 0.416 & 0.807 & 0.445 & 0.818 \\
                BAE-MCD & 0.607 & 0.786 & 0.584 & 0.833 \\
                BAE-BBB & 0.675 & 0.805 & 0.659 & 0.829 \\
                BAE-Ensemble & 0.708 & \textbf{0.844} & 0.702 & 0.832 \\ \midrule
                \textbf{Mean} & 0.618 & 0.815 & 0.610 & 0.825 \\ \bottomrule
                \end{tabular}
            }
       
     \end{subtable}
     
     \label{table:retained}
\end{table}

% BAE-\scalebox{1.25}{$\infty$} & - & - & 0.856 & \textbf{0.858} \\ \midrule

% \begin{tabular}{@{}lcccc@{}}
% \toprule
%  & \multicolumn{1}{c}{Bottleneck} & \multicolumn{3}{c}{--Without Bottleneck--} \\ \midrule
% \multicolumn{1}{c}{Model} & \multicolumn{1}{c}{A} & \multicolumn{1}{c}{B} & \multicolumn{1}{c}{C} & \multicolumn{1}{c}{D} \\ \midrule

==> tables/FashionMNIST_bottleneck.tex <==
\begin{table}[H] 
\caption{AUROC scores for deterministic AE, VAE and BAE-Ensemble with various architectures (type A, B, C or D) are categorised as either with a bottleneck or without. The model scoring the highest AUROC is bolded. The mean treatment effects of removing the bottleneck are quantified in the last row.}

% \begin{subtable}[h]{\textwidth}
%     \centering
%     \scriptsize \caption{ZEMA}
%         \resizebox{0.8\textwidth}{!}{
%             \begin{tabular}{@{}lcccc@{}}
%             \toprule
%              & ---Bottleneck--- & \multicolumn{3}{c}{------------------Without Bottleneck------------------} \\ 
%              \multicolumn{1}{c}{Model} & \begin{tabular}[c]{@{}c@{}}A\\ Undercomplete\\ No skip\end{tabular} & \begin{tabular}[c]{@{}c@{}}B\\ Undercomplete\\ + skip\end{tabular} & \begin{tabular}[c]{@{}c@{}}C\\ Overcomplete\\ No skip\end{tabular} & \begin{tabular}[c]{@{}c@{}}D\\ Overcomplete\\ + skip\end{tabular} \\ \midrule

%             % \multicolumn{1}{c}{Model} & \begin{tabular}[c]{@{}c@{}}A\\ Undercomplete\\ No skip\end{tabular} & \begin{tabular}[c]{@{}c@{}}B\\ Undercomplete\\ +skip\end{tabular} & \begin{tabular}[c]{@{}c@{}}C\\ Overcomplete\\ No skip\end{tabular} & \begin{tabular}[c]{@{}c@{}}D\\ Overcomplete\\ +skip\end{tabular} \\ \midrule

%             Deterministic AE & 0.906 & 0.943 & 0.925 & 0.947 \\
%             VAE & 0.895 & 0.938 & 0.892 & 0.947 \\
%             BAE-MCD & 0.901 & 0.937 & 0.898 & 0.942 \\
%             BAE-BBB & 0.900 & 0.947 & 0.907 & 0.936 \\ 
%             BAE-Ensemble & 0.944 & 0.964 & 0.929 & 0.965 \\ 
%             BAE-\scalebox{1.25}{$\infty$}  & - & - & 0.968 & \textbf{0.992} \\ \midrule
%             \textbf{Mean} & 0.909 & 0.946 & 0.920 & 0.955 \\ \bottomrule
%             \end{tabular}
%         }
% \end{subtable}
% \hfill
    \begin{subtable}[h]{\textwidth}
        \centering
        \vskip 0.2in
        \scriptsize \caption{FashionMNIST vs MNIST}
            \resizebox{0.8\textwidth}{!}{
                \begin{tabular}{@{}lcccc@{}}
                \toprule
                 & ---Bottleneck--- & \multicolumn{3}{c}{------------------Without Bottleneck------------------} \\ 
                 \multicolumn{1}{c}{Model} & \begin{tabular}[c]{@{}c@{}}A\\ Undercomplete\\ No skip\end{tabular} & \begin{tabular}[c]{@{}c@{}}B\\ Undercomplete\\ + skip\end{tabular} & \begin{tabular}[c]{@{}c@{}}C\\ Overcomplete\\ No skip\end{tabular} & \begin{tabular}[c]{@{}c@{}}D\\ Overcomplete\\ + skip\end{tabular} \\ \midrule

Deterministic AE & 0.993 & 0.951 & 0.985 & 0.926 \\
VAE & 0.839 & 0.939 & 0.929 & 0.825 \\
BAE-MCD & 0.986 & 0.703 & 0.986 & 0.866 \\
BAE-BBB & \textbf{0.994} & 0.788 & \textbf{0.994} & 0.942 \\
BAE-Ensemble & 0.990 & 0.933 & 0.984 & 0.929 \\ \midrule
\textbf{Mean} & 0.960 & 0.863 & 0.976 & 0.898 \\ \bottomrule
                \end{tabular}
            }
       
     \end{subtable}
     
     \label{table:retained}
\end{table}

% BAE-\scalebox{1.25}{$\infty$} & - & - & 0.856 & \textbf{0.858} \\ \midrule

% \begin{tabular}{@{}lcccc@{}}
% \toprule
%  & \multicolumn{1}{c}{Bottleneck} & \multicolumn{3}{c}{--Without Bottleneck--} \\ \midrule
% \multicolumn{1}{c}{Model} & \multicolumn{1}{c}{A} & \multicolumn{1}{c}{B} & \multicolumn{1}{c}{C} & \multicolumn{1}{c}{D} \\ \midrule

==> tables/FashionMNIST_table.tex <==
%Table 1 - FashionMNIST vs MNIST
\begin{table}[!ht]
\centering
\caption{(FashionMNIST vs MNIST) AUROC for detecting OOD inputs with deterministic AE, VAE and BAE (MC-Dropout, Bayes by Backprop and anchored ensembling) with posterior approximated under various techniques. For each likelihood- Bernoulli, Continuous Bernoulli and Gaussian, we compare the performance of using $\mathrm{Var}_\theta(\hat{\textbf{x}})$, $\E_{\theta}\mathrm{(LL)}$, $\mathrm{Var_{\theta}(LL)}$, and WAIC. Results where AUROC\textgreater{0.8} are in bold.}
\label{table-results-fashionMNIST}

\resizebox{.65\textwidth}{!}{
\begin{tabular}{@{}llcccc@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Model}} & \multicolumn{1}{c}{\multirow{2}{*}{Likelihood}} & \multicolumn{4}{c}{AUROC}                                  \\ \cmidrule(l){3-6} 
\multicolumn{1}{c}{}                       & \multicolumn{1}{c}{}                            & $\mathrm{Var}_\theta(\hat{\textbf{x}}^*)$ & $\E_{\theta}\mathrm{(LL)}$ & $\mathrm{Var_{\theta}(LL)}$ & WAIC \\ \midrule
Deterministic AE                                         & Ber($\hat{{x}}^*$)                                             & -                & 0.230       & -           & -           \\
Deterministic AE                                         & C-Ber($\hat{{x}}^*$)                                           & -                & 0.203       & -           & -           \\
Deterministic AE                                         & N($\hat{{x}}^*$,1)                                               & -                & \textbf{0.978}       & -           & -           \\ \midrule
VAE                                        & Ber($\hat{{x}}^*$)                                             & 0.629            & 0.393       & \textbf{0.982}       & 0.454       \\
VAE                                        & C-Ber($\hat{{x}}^*$)                                           & 0.365            & 0.301       & \textbf{0.995}       & 0.389       \\
VAE                                        & N($\hat{{x}}^*$,1)                                               & 0.420            & \textbf{0.987}       & \textbf{0.948}       & \textbf{0.987}      \\ \midrule
BAE, MC-Dropout                            & Ber($\hat{{x}}^*$)                                             & 0.610            & 0.224       & \textbf{0.983}       & 0.250       \\
BAE, MC-Dropout                            & C-Ber($\hat{{x}}^*$)                                           & 0.670            & 0.183       & \textbf{0.981}       & 0.237       \\
BAE, MC-Dropout                            & N($\hat{{x}}^*$,1)                                               & \textbf{0.820}            & \textbf{0.977}  & \textbf{0.991}       & \textbf{0.978}       \\ \midrule
BAE, BayesBB                                    & Ber($\hat{{x}}^*$)                                             & 0.736            & 0.258       & \textbf{0.987}       & 0.371       \\
BAE, BayesBB                                    & C-Ber($\hat{{x}}^*$)                                           & 0.750            & 0.204       & \textbf{0.991}       & 0.308       \\
BAE, BayesBB                                    & N($\hat{{x}}^*$,1)                                               & 0.701            & \textbf{0.945}       & \textbf{0.941}       & \textbf{0.951}       \\ \midrule
BAE, Ensemble                              & Ber($\hat{{x}}^*$)                                             & \textbf{0.990}            & 0.230       & \textbf{0.999}       & 0.314       \\
BAE, Ensemble                              & C-Ber($\hat{{x}}^*$)                                           & \textbf{0.978}            & 0.191       & \textbf{0.999}       & 0.418       \\
BAE, Ensemble                              & N($\hat{{x}}^*$,1)                                               & \textbf{0.995}            & \textbf{0.976}       & \textbf{0.998}       & \textbf{0.980}       \\ \bottomrule
\end{tabular}
}
\end{table}


==> tables/MNIST_table.tex <==
%Table 2 - MNIST
\begin{table}[ht]
\caption{(MNIST vs FashionMNIST) AUROC for various models and likelihoods. Results where AUROC\textgreater{0.8} are in bold.}
\label{table-results-MNIST}
\resizebox{.65\textwidth}{!}{
\begin{tabular}{@{}llcccc@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Model}} & \multicolumn{1}{c}{\multirow{2}{*}{Likelihood}} & \multicolumn{4}{c}{AUROC}                                  \\ \cmidrule(l){3-6} 
\multicolumn{1}{c}{}                       & \multicolumn{1}{c}{}                            & $\mathrm{Var}_\theta(\hat{\textbf{x}}^*)$ & $\E_{\theta}\mathrm{(LL)}$ & $\mathrm{Var_{\theta}(LL)}$ & WAIC \\ \midrule
Deterministic AE                                         & Ber($\hat{x}^*$)                                             & -                & \textbf{1.00}        & -           & -           \\
Deterministic AE                                         & C-Ber($\hat{x}^*$)                                           & -                & \textbf{1.00}        & -           & -           \\
Deterministic AE                                         & N($\hat{x}^*$,1)                                               & -                & \textbf{0.999}       & -           & -           \\ \midrule
VAE                                        & Ber($\hat{x}^*$)                                             & \textbf{0.996}            & \textbf{1.00}        & \textbf{1.00}        & \textbf{1.00}        \\
VAE                                        & C-Ber($\hat{x}^*$)                                           & \textbf{0.990}            & \textbf{1.00}        & \textbf{0.997}       & \textbf{1.00}        \\
VAE                                        & N($\hat{x}^*$,1)                                               & \textbf{0.973}            & \textbf{0.999}       & \textbf{0.982}       & \textbf{0.999}       \\ \midrule
BAE, MC-Dropout                            & Ber($\hat{x}^*$)                                             & 0.600            & \textbf{1.00}        & \textbf{0.995}       & \textbf{1.00}        \\
BAE, MC-Dropout                            & C-Ber($\hat{x}^*$)                                           & 0.713            & \textbf{1.00}        & \textbf{0.930}       & \textbf{0.999}       \\
BAE, MC-Dropout                            & N($\hat{x}^*$,1)                                               & 0.331            & \textbf{0.999}       & 0.636       & \textbf{0.999}       \\ \midrule
BAE, BayesBB                                    & Ber($\hat{x}^*$)                                             & \textbf{0.834}            & \textbf{0.998}       & \textbf{0.885}       & \textbf{0.921}       \\
BAE, BayesBB                                    & C-Ber($\hat{x}^*$)                                           & \textbf{0.864}            & \textbf{0.990}       & 0.714       & \textbf{0.904}       \\
BAE, BayesBB                                    & N($\hat{x}^*$,1)                                               & \textbf{0.859}            & \textbf{0.998}       & \textbf{0.863}       & \textbf{0.998}       \\ \midrule
BAE, Ensemble                              & Ber($\hat{x}^*$)                                             & \textbf{0.995}            & \textbf{1.00}        & \textbf{0.999}       & \textbf{1.00}        \\
BAE, Ensemble                              & C-Ber($\hat{x}^*$)                                           & \textbf{0.996}            & \textbf{1.00}        & \textbf{0.997}       & \textbf{1.00}        \\
BAE, Ensemble                              & N($\hat{x}^*$,1)                                               & \textbf{0.996}            & \textbf{0.999}       & \textbf{0.991}       & \textbf{0.999}       \\ \bottomrule
\end{tabular}
}
\end{table}

==> tables/STRATH_LL.tex <==
%Table 1 - FashionMNIST vs MNIST
\begin{table}[!ht]
\centering
\caption{(STRATH) AUROC for detecting OOD inputs with deterministic AE, VAE and BAE (MC-Dropout, Bayes by Backprop and anchored ensembling) with posterior approximated under various techniques. For each likelihood- Bernoulli, Continuous Bernoulli and Gaussian, we compare the performance of using $\mathrm{Var}_\theta(\hat{\textbf{x}})$, $\E_{\theta}\mathrm{(LL)}$, $\mathrm{Var_{\theta}(LL)}$, and WAIC. Results where AUROC\textgreater{0.8} are in bold.}
\label{table-results-fashionMNIST}

\resizebox{.65\textwidth}{!}{
\begin{tabular}{@{}llcccc@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Model}} & \multicolumn{1}{c}{\multirow{2}{*}{Likelihood}} & \multicolumn{4}{c}{AUROC}                                  \\ \cmidrule(l){3-6} 
\multicolumn{1}{c}{}                       & \multicolumn{1}{c}{}                            & $\mathrm{Var}_\theta(\hat{\textbf{x}}^*)$ & $\E_{\theta}\mathrm{(LL)}$ & $\mathrm{Var_{\theta}(LL)}$ & WAIC \\ \midrule
Deterministic AE & Ber($\hat{{x}}^*$) & - & 0.310 & - & - \\
Deterministic AE & C-Ber($\hat{{x}}^*$) & - & 0.286 & - & - \\
Deterministic AE & N($\hat{{x}}^*$,1) & - & \textbf{0.862} & - & - \\ \midrule
VAE & Ber($\hat{{x}}^*$) & 0.519 & 0.404 & 0.723 & 0.404 \\
VAE & C-Ber($\hat{{x}}^*$) & 0.496 & 0.382 & 0.730 & 0.382 \\
VAE & N($\hat{{x}}^*$,1) & 0.511 & \textbf{0.863} & 0.707 & \textbf{0.863} \\ \midrule
BAE-MCD & Ber($\hat{{x}}^*$) & 0.501 & 0.370 & 0.573 & 0.370 \\
BAE-MCD & C-Ber($\hat{{x}}^*$) & 0.554 & 0.284 & 0.607 & 0.284 \\
BAE-MCD & N($\hat{{x}}^*$,1) & 0.505 & \textbf{0.867} & 0.588 & \textbf{0.867} \\ \midrule
BAE-BBB & Ber($\hat{{x}}^*$) & 0.523 & 0.361 & 0.663 & 0.361 \\
BAE-BBB & C-Ber($\hat{{x}}^*$) & 0.559 & 0.312 & 0.629 & 0.312 \\
BAE-BBB & N($\hat{{x}}^*$,1) & 0.528 & \textbf{0.854} & 0.675 & \textbf{0.854} \\ \midrule
BAE-Ensemble & Ber($\hat{{x}}^*$) & 0.638 & 0.364 & 0.682 & 0.364 \\
BAE-Ensemble & C-Ber($\hat{{x}}^*$) & 0.633 & 0.298 & 0.674 & 0.298 \\
BAE-Ensemble & N($\hat{{x}}^*$,1) & 0.623 & \textbf{0.868} & 0.708 & \textbf{0.868} \\ \bottomrule
\end{tabular}
}
\end{table}


==> tables/SVHN_table.tex <==
%Table 3 - SVHN
\begin{table}[ht]
\caption{(SVHN vs CIFAR10) AUROC for various models and likelihoods. Results where AUROC\textgreater{0.8} are in bold.}
\label{table-results-SVHN}
\resizebox{.65\textwidth}{!}{
\begin{tabular}{@{}llcccc@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Model}} & \multicolumn{1}{c}{\multirow{2}{*}{Likelihood}} & \multicolumn{4}{c}{AUROC}                                  \\ \cmidrule(l){3-6} 
\multicolumn{1}{c}{}                       & \multicolumn{1}{c}{}                            & $\mathrm{Var_\theta(\hat{\textbf{x}}^*)}$ & $\E_{\theta}\mathrm{(LL)}$ & $\mathrm{Var_{\theta}(LL)}$ & WAIC \\ \midrule
Deterministic AE                                         & Ber($\hat{x}^*$)                                              & -                & 0.442       & -           & -           \\
Deterministic AE                                         & C-Ber($\hat{x}^*$)                                           & -                & 0.436       & -           & -           \\
Deterministic AE                                         & N($\hat{x}^*$,1)                                               & -                & \textbf{0.972}       & -           & -           \\ \midrule
VAE                                        & Ber($\hat{x}^*$)                                             & 0.751            & 0.455       & \textbf{0.948}       & 0.456       \\
VAE                                        & C-Ber($\hat{x}^*$)                                           & 0.526            & 0.435       & \textbf{0.947}       & 0.436       \\
VAE                                        & N($\hat{x}^*$,1)                                               & 0.630            & \textbf{0.973}       & \textbf{0.964}       & \textbf{0.973}       \\ \midrule
BAE, MC-Dropout                            & Ber($\hat{x}^*$)                                             & \textbf{0.820}            & 0.445       & \textbf{0.923}       & 0.446       \\
BAE, MC-Dropout                            & C-Ber($\hat{x}^*$)                                           & \textbf{0.861}            & 0.441       & \textbf{0.898}       & 0.445       \\
BAE, MC-Dropout                            & N($\hat{x}^*$,1)                                               & \textbf{0.802}            & \textbf{0.967}       & \textbf{0.938}       & \textbf{0.967}       \\ \midrule
BAE, BayesBB                                    & Ber($\hat{x}^*$)                                             & 0.649            & 0.570       & 0.797       & 0.606       \\
BAE, BayesBB                                    & C-Ber($\hat{x}^*$)                                           & \textbf{0.855}            & 0.485       & \textbf{0.877}       & 0.502       \\
BAE, BayesBB                                    & N($\hat{x}^*$,1)                                               & 0.760            & \textbf{0.918}       & \textbf{0.851}       & \textbf{0.915}       \\ \midrule
BAE, Ensemble                              & Ber($\hat{x}^*$)                                             & \textbf{0.922}            & 0.440       & \textbf{0.950}       & 0.441       \\
BAE, Ensemble                              & C-Ber($\hat{x}^*$)                                           & \textbf{0.921}            & 0.436       & \textbf{0.939}       & 0.439       \\
BAE, Ensemble                              & N($\hat{x}^*$,1)                                               & \textbf{0.931}            & \textbf{0.969}       & \textbf{0.960}       & \textbf{0.969}       \\ \bottomrule
\end{tabular}
}
\end{table}

==> tables/ZEMA_LL.tex <==
% ZEMA
\begin{table}[!ht]
\centering
\caption{(ZEMA) AUROC for detecting OOD inputs with deterministic AE, VAE and BAE (MC-Dropout, Bayes by Backprop and anchored ensembling) with posterior approximated under various techniques. For each likelihood- Bernoulli, Continuous Bernoulli and Gaussian, we compare the performance of using $\mathrm{Var}_\theta(\hat{\textbf{x}})$, $\E_{\theta}\mathrm{(LL)}$, $\mathrm{Var_{\theta}(LL)}$, and WAIC. Results where AUROC\textgreater{0.8} are in bold.}
\label{table-results-fashionMNIST}

\resizebox{.65\textwidth}{!}{
\begin{tabular}{@{}llcccc@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Model}} & \multicolumn{1}{c}{\multirow{2}{*}{Likelihood}} & \multicolumn{4}{c}{AUROC}                                  \\ \cmidrule(l){3-6} 
\multicolumn{1}{c}{}                       & \multicolumn{1}{c}{}                            & $\mathrm{Var}_\theta(\hat{\textbf{x}}^*)$ & $\E_{\theta}\mathrm{(LL)}$ & $\mathrm{Var_{\theta}(LL)}$ & WAIC \\ \midrule
Deterministic AE & Ber($\hat{{x}}^*$) & - & 0.570 &- & - \\
Deterministic AE & C-Ber($\hat{{x}}^*$) & - & 0.581 & - & - \\
Deterministic AE & N($\hat{{x}}^*$,1) & - & \textbf{0.918} & - & - \\ \midrule
VAE & Ber($\hat{{x}}^*$) & 0.500 & 0.568 & 0.716 & 0.568 \\
VAE & C-Ber($\hat{{x}}^*$) & 0.491 & 0.593 & \textbf{0.862} & 0.593 \\
VAE & N($\hat{{x}}^*$,1) & 0.539 & \textbf{0.911} & 0.714 & \textbf{0.911} \\ \midrule
BAE-MCD & Ber($\hat{{x}}^*$) & 0.461 & 0.566 & 0.643 & 0.566 \\
BAE-MCD & C-Ber($\hat{{x}}^*$) & 0.565 & 0.582 & 0.761 & 0.582 \\
BAE-MCD & N($\hat{{x}}^*$,1) & 0.509 & \textbf{0.904} & 0.649 & \textbf{0.904} \\ \midrule
BAE-BBB & Ber($\hat{{x}}^*$) & 0.430 & 0.576 & \textbf{0.931} & 0.576 \\
BAE-BBB & C-Ber($\hat{{x}}^*$) & 0.474 & 0.584 & \textbf{0.904} & 0.584 \\
BAE-BBB & N($\hat{{x}}^*$,1) & 0.493 & \textbf{0.933} & \textbf{0.914} & \textbf{0.933} \\ \midrule
BAE-Ensemble & Ber($\hat{{x}}^*$) & 0.78 & 0.569 & \textbf{0.823} & 0.569 \\
BAE-Ensemble & C-Ber($\hat{{x}}^*$) & 0.754 & 0.584 & \textbf{0.853} & 0.584 \\
BAE-Ensemble & N($\hat{{x}}^*$,1) & \textbf{0.810} & \textbf{0.963} & \textbf{0.905} & \textbf{0.963} \\ \bottomrule
\end{tabular}
}
\end{table}


==> tables/ZEMA_bottleneck.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \begin{table}[!ht]
% \centering
%     \begin{tabular}{@{}lcccc@{}}
%     \toprule
%      & Bottleneck & \multicolumn{3}{c}{--Without Bottleneck--} \\
%     \multicolumn{1}{c}{Model} & A & B & C & D \\ \midrule
%     Deterministic AE & 0.923 & 0.892 & 0.936 & 0.929 \\
%     BAE-Ensemble & 0.948 & 0.942 & \textbf{0.966} & 0.963 \\
%     VAE & 0.897 & 0.905 & 0.936 & 0.933 \\ \midrule
%     Mean & 0.923 & 0.913 & 0.946 & 0.942 \\ \bottomrule
%     \end{tabular}
% \end{table}

% \begin{table}[!ht]
% \centering
%     \begin{tabular}{@{}lcccc@{}}
%     \toprule
%      & Bottleneck & \multicolumn{3}{c}{--Without Bottleneck--} \\
%     \multicolumn{1}{c}{Model} & A & B & C & D \\ \midrule
%     Deterministic AE & 0.923 & 0.892 & 0.936 & 0.929 \\
%     BAE-Ensemble & 0.948 & 0.942 & \textbf{0.966} & 0.963 \\
%     VAE & 0.897 & 0.905 & 0.936 & 0.933 \\ \midrule
%     Mean & 0.923 & 0.913 & 0.946 & 0.942 \\ \bottomrule
%     \end{tabular}
% \end{table}


\begin{table}[H] 
\caption{AUROC scores for deterministic AE, VAE and BAE-Ensemble with various architectures (type A, B, C or D) are categorised as either with a bottleneck or without. For each dataset, the model scoring the highest AUROC is bolded.}

    \begin{subtable}[h]{\textwidth}
        \centering
        \scriptsize \caption{ZEMA}
            \resizebox{0.8\textwidth}{!}{
                \begin{tabular}{@{}lcccc@{}}
                \toprule
                 & ---Bottleneck--- & \multicolumn{3}{c}{------------------Without Bottleneck------------------} \\ 
                 \multicolumn{1}{c}{Model} & \begin{tabular}[c]{@{}c@{}}A\\ Undercomplete\\ No skip\end{tabular} & \begin{tabular}[c]{@{}c@{}}B\\ Undercomplete\\ + skip\end{tabular} & \begin{tabular}[c]{@{}c@{}}C\\ Overcomplete\\ No skip\end{tabular} & \begin{tabular}[c]{@{}c@{}}D\\ Overcomplete\\ + skip\end{tabular} \\ \midrule

                % \multicolumn{1}{c}{Model} & \begin{tabular}[c]{@{}c@{}}A\\ Undercomplete\\ No skip\end{tabular} & \begin{tabular}[c]{@{}c@{}}B\\ Undercomplete\\ +skip\end{tabular} & \begin{tabular}[c]{@{}c@{}}C\\ Overcomplete\\ No skip\end{tabular} & \begin{tabular}[c]{@{}c@{}}D\\ Overcomplete\\ +skip\end{tabular} \\ \midrule

                Deterministic AE & 0.906 & 0.943 & 0.925 & 0.947 \\
                VAE & 0.895 & 0.938 & 0.892 & 0.947 \\
                BAE-MCD & 0.901 & 0.937 & 0.898 & 0.942 \\
                BAE-BBB & 0.900 & 0.947 & 0.907 & 0.936 \\ 
                BAE-Ensemble & 0.944 & 0.964 & 0.929 & 0.965 \\ 
                BAE-\scalebox{1.25}{$\infty$}  & - & - & 0.968 & \textbf{0.992} \\ \midrule
                \textbf{Mean} & 0.909 & 0.946 & 0.920 & 0.955 \\ \bottomrule
                \end{tabular}
            }
       
    \end{subtable}
    \hfill
    \begin{subtable}[h]{\textwidth}
        \centering
        \vskip 0.2in
        \scriptsize \caption{STRATH}
            \resizebox{0.8\textwidth}{!}{
                \begin{tabular}{@{}lcccc@{}}
                \toprule
                 & ---Bottleneck--- & \multicolumn{3}{c}{------------------Without Bottleneck------------------} \\ 
                 \multicolumn{1}{c}{Model} & \begin{tabular}[c]{@{}c@{}}A\\ Undercomplete\\ No skip\end{tabular} & \begin{tabular}[c]{@{}c@{}}B\\ Undercomplete\\ + skip\end{tabular} & \begin{tabular}[c]{@{}c@{}}C\\ Overcomplete\\ No skip\end{tabular} & \begin{tabular}[c]{@{}c@{}}D\\ Overcomplete\\ + skip\end{tabular} \\ \midrule

                Deterministic AE & 0.837 & 0.813 & 0.827 & 0.833 \\
                VAE & 0.828 & 0.850 & 0.836 & 0.837 \\
                BAE-MCD & 0.849 & 0.823 & 0.842 & 0.825 \\
                BAE-BBB & 0.850 & 0.840 & 0.849 & 0.841 \\ 
                BAE-Ensemble & 0.840 & 0.856 & 0.837 & \textbf{0.858} \\ 
                BAE-\scalebox{1.25}{$\infty$}  & - & - & 0.811 & 0.789 \\ \midrule
                \textbf{Mean} & 0.841 & 0.837 & 0.834 & 0.831 \\ \bottomrule
                \end{tabular}
            }
       
     \end{subtable}
     
     \label{table:retained}
\end{table}

% BAE-\scalebox{1.25}{$\infty$} & - & - & 0.856 & \textbf{0.858} \\ \midrule

% \begin{tabular}{@{}lcccc@{}}
% \toprule
%  & \multicolumn{1}{c}{Bottleneck} & \multicolumn{3}{c}{--Without Bottleneck--} \\ \midrule
% \multicolumn{1}{c}{Model} & \multicolumn{1}{c}{A} & \multicolumn{1}{c}{B} & \multicolumn{1}{c}{C} & \multicolumn{1}{c}{D} \\ \midrule

==> tables/bottleneck_full_perc.tex <==
\begin{table}[hbtp]
\caption{AUROC scores for deterministic AE, VAE and BAEs with and without a bottleneck. Model with highest AUROC is bolded for each dataset.}
\centering
\resizebox{.78\textwidth}{!}{
\begin{tabular}{@{}lcccc@{}}
                \toprule
                 & ---Bottleneck--- & \multicolumn{3}{c}{------------------Without bottleneck------------------} \\ 
                 \multicolumn{1}{c}{Model} & \begin{tabular}[c]{@{}c@{}}A\\ Undercomplete\\ No skip\end{tabular} & \begin{tabular}[c]{@{}c@{}}B\\ Undercomplete\\ + skip\end{tabular} & \begin{tabular}[c]{@{}c@{}}C\\ Overcomplete\\ No skip\end{tabular} & \begin{tabular}[c]{@{}c@{}}D\\ Overcomplete\\ + skip\end{tabular} \\ \midrule

\multicolumn{5}{l}{\textbf{FashionMNIST vs MNIST}, four runs} \\
\,\quad Deterministic AE & 98.6\,$\pm$\,0.3 & 91.2\,$\pm$\,4.5 & 97.6\,$\pm$\,0.4 & 85.8\,$\pm$\,3.7 \\
\,\quad VAE & 79.3\,$\pm$\,3.6 & 89.5\,$\pm$\,4.8 & 91.3\,$\pm$\,1.4 & 88.4\,$\pm$\,2.9 \\
\,\quad BAE-MCD & 98.3\,$\pm$\,0.1 & 71.2\,$\pm$\,3.5 & 98.4\,$\pm$\,0.1 & 78.3\,$\pm$\,0.6 \\
\,\quad BAE-BBB & \textbf{99.2\,$\pm$\,0.6} & 84.8\,$\pm$\,4.8 & 99.0\,$\pm$\,0.1 & 90.1\,$\pm$\,1.8 \\
\,\quad BAE-Ensemble & 98.5\,$\pm$\,0.0 & 92.0\,$\pm$\,0.1 & 97.7\,$\pm$\,0.1 & 92.8\,$\pm$\,0.2 \\
\,\quad BAE-\scalebox{1.25}{$\infty$}& - & - & 93.0\,$\pm$\,0.2 & - \\
\multicolumn{5}{l}{\textbf{CIFAR vs SVHN}, four runs} \\
\,\quad Deterministic AE & 68.6\,$\pm$\,1.1 & 81.6\,$\pm$\,0.2 & 69.2\,$\pm$\,1.3 & 82.0\,$\pm$\,1.6 \\
\,\quad VAE & 39.8\,$\pm$\,1.4 & 82.2\,$\pm$\,0.6 & 42.8\,$\pm$\,0.8 & 84.0\,$\pm$\,0.6 \\
\,\quad BAE-MCD & 61.3\,$\pm$\,0.7 & 80.9\,$\pm$\,1.9 & 62.6\,$\pm$\,0.1 & 83.4\,$\pm$\,0.4 \\
\,\quad BAE-BBB & 67.2\,$\pm$\,0.6 & 83.1\,$\pm$\,3.0 & 63.9\,$\pm$\,1.4 & 82.6\,$\pm$\,0.2 \\
\,\quad BAE-Ensemble & 69.6\,$\pm$\,2.0 & \textbf{84.9\,$\pm$\,1.1} & 69.9\,$\pm$\,2.4 & 83.8\,$\pm$\,0.9 \\
\,\quad BAE-\scalebox{1.25}{$\infty$} & - & - & 77.1\,$\pm$\,0.1 & - \\
\multicolumn{5}{l}{\textbf{ODDS}, eight datasets, ten runs} \\
\,\quad Deterministic AE & 81.9\,$\pm$\,1.4 & 87.2\,$\pm$\,1.1 & 83.3\,$\pm$\,1.3 & 84.8\,$\pm$\,1.2 \\
\,\quad VAE & 79.5\,$\pm$\,1.4 & 87.6\,$\pm$\,0.8 & 81.9\,$\pm$\,1.3 & 88.3\,$\pm$\,0.8 \\
\,\quad BAE-MCD & 82.9\,$\pm$\,1.5 & 89.1\,$\pm$\,1.0 & 81.9\,$\pm$\,1.3 & 85.6\,$\pm$\,1.1 \\
\,\quad BAE-BBB & 89.2\,$\pm$\,1.1 & 91.3\,$\pm$\,0.7 & \textbf{91.9\,$\pm$\,0.7} & 91.7\,$\pm$\,0.7 \\
\,\quad BAE-Ensemble & 85.7\,$\pm$\,1.2 & 88.6\,$\pm$\,1.0 & 85.0\,$\pm$\,1.1 & 86.0\,$\pm$\,1.2 \\
\,\quad BAE-\scalebox{1.25}{$\infty$} & - & - & 91.3\,$\pm$\,1.3 & - \\
\multicolumn{5}{l}{\textbf{ZeMA}, four tasks, ten runs} \\
\,\quad Deterministic AE & 87.9\,$\pm$\,2.4 & 93.0\,$\pm$\,1.0 & 91.1\,$\pm$\,1.4 & 90.8\,$\pm$\,1.9 \\
\,\quad VAE & 87.9\,$\pm$\,1.5 & 91.7\,$\pm$\,1.6 & 87.6\,$\pm$\,1.9 & 92.2\,$\pm$\,1.6 \\
\,\quad BAE-MCD & 89.2\,$\pm$\,1.7 & 92.0\,$\pm$\,1.5 & 86.2\,$\pm$\,2.3 & 93.6\,$\pm$\,0.8 \\
\,\quad BAE-BBB & 88.8\,$\pm$\,1.9 & 93.9\,$\pm$\,0.7 & 89.5\,$\pm$\,1.9 & 93.1\,$\pm$\,0.9 \\
\,\quad BAE-Ensemble & 93.8\,$\pm$\,0.7 & 96.1\,$\pm$\,0.5 & 92.8\,$\pm$\,0.7 & \textbf{96.3\,$\pm$\,0.4} \\
\,\quad BAE-\scalebox{1.25}{$\infty$} & - & - & 92.6\,$\pm$\,1.0 & - \\
\multicolumn{5}{l}{\textbf{STRATH}, four tasks, ten runs} \\
\,\quad Deterministic AE & 81.7\,$\pm$\,1.0 & 81.1\,$\pm$\,1.5 & 81.9\,$\pm$\,1.0 & 81.9\,$\pm$\,1.2 \\
\,\quad VAE & 82.5\,$\pm$\,0.9 & 83.1\,$\pm$\,1.2 & 83.1\,$\pm$\,0.8 & 82.4\,$\pm$\,1.4 \\
\,\quad BAE-MCD & 83.8\,$\pm$\,0.8 & 80.8\,$\pm$\,1.6 & 83.8\,$\pm$\,0.7 & 82.2\,$\pm$\,1.4 \\
\,\quad BAE-BBB & 84.7\,$\pm$\,0.8 & 83.4\,$\pm$\,0.7 & 84.8\,$\pm$\,0.8 & 83.3\,$\pm$\,0.8 \\
\,\quad BAE-Ensemble & 83.9\,$\pm$\,0.8 & 85.0\,$\pm$\,0.7 & 83.5\,$\pm$\,0.7 & \textbf{85.5\,$\pm$\,0.6} \\
\,\quad BAE-\scalebox{1.25}{$\infty$} & - & - & 71.7\,$\pm$\,0.9 & - \\ \hline
\quad \textbf{Mean} & 82.5\,$\pm$\,1.2 & 86.6\,$\pm$\,1.6 & 83.5\,$\pm$\,1.0 & \textbf{86.7\,$\pm$\,1.2} \\
\quad \textbf{ATE} & - & 4.1 & 1.0 & \textbf{4.2} \\ \hline

\end{tabular}
}
\label{table:btneck-res}
\end{table}

==> tables/fmnist_cifar_architectures.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[H]
\caption{Encoder architectures for FashionMNIST, MNIST, CIFAR10 and SVHN acting as in-distribution training dataset. The decoder is a reflection of the encoder, in which the convolution layers are replaced by convolution transpose layers.}
\label{table-architecture}
\centering
\vskip 0.1in
a) FashionMNIST vs MNIST
\begin{tabular}{@{}cccc@{}}
\toprule
Layer       & Output dimensions & Kernel & Strides \\ \midrule
Convolution & 13 x 13 x 32      & 4 x 4  & 2 x 2   \\
Convolution & 10 x 10 x 64      & 4 x 4  & 1 x 1   \\
Reshape     & 6400              & -      & -       \\
Dense       & Latent size       & -      & -      \\ \bottomrule
\end{tabular}
\newline \newline
b) CIFAR10 vs SVHN
\begin{tabular}{@{}cccc@{}}
\toprule
Layer       & Output dimensions & Kernel & Strides \\ \midrule
Convolution & 15 x 15 x 32      & 4 x 4  & 2 x 2   \\
Convolution & 12 x 12 x 64      & 4 x 4  & 1 x 1   \\
Convolution & 5 x 5 x 128       & 4 x 4  & 2 x 2   \\
Reshape     & 3200              & -      & -       \\
Dense       & Latent size       & -      & -      \\ \bottomrule
\end{tabular}
\end{table}



==> tables/zema_strath_odds_architecture.tex <==
\begin{table}[h] 
\centering
\caption{Encoder architecture for ODDS, ZeMA and STRATH datasets. We set the latent dimensions to be half of the flattened input dimensions. The decoder is a reflection of the encoder, in which the Conv1D layers are replaced by Conv1D-Transpose layers. We apply layer normalisation after each Conv1D and linear layer for ODDS and STRATH. The leaky ReLu \cite{maas2013rectifier} is used as the activation function with a slope of 0.01 while the sigmoid function is used at the decoder's final layer.}


    \begin{subtable}[h]{\textwidth}
        \centering
        \scriptsize \caption{ODDS}
            \resizebox{0.6\textwidth}{!}{
                    \begin{tabular}{@{}cccc@{}}
                    \toprule
                    Layer       & Output channels/nodes & Kernel & Strides \\ \midrule
                    Linear       & Input dimensions $\times 4$      & -      & -      \\ 
                    Linear       & Input dimensions $\times 4$       & -      & -      \\ 
                    Linear       & Latent dimensions       & -      & -      \\ \bottomrule
                    \end{tabular}
            }
    \end{subtable}
    \hfill
    \begin{subtable}[h]{0.6\textwidth}
        \centering
        \vskip 0.2in
        \scriptsize \caption{ZeMA and STRATH}
            \resizebox{\textwidth}{!}{
                \begin{tabular}{@{}cccc@{}}
                \toprule
                Layer       & Output channels/nodes & Kernel & Strides \\ \midrule
                Conv1D & 10      & 8  & 2   \\
                Conv1D & 20      & 2  & 2   \\
                Reshape     & -              & -      & -       \\
                Linear       & 1000       & -      & -      \\ 
                Linear       & Latent dimensions       & -      & -      \\ \bottomrule
                \end{tabular}
            }
    \end{subtable}
     \label{table:architecture}
\end{table}



